ULEEN: A Novel Architecture for Ultra Low-Energy Edge Neural Networks

The deployment of AI models on low-power, real-time edge devices requires accelerators for which energy, latency, and area are all first-order concerns. There are many approaches to enabling deep neural networks (DNNs) in this domain, including pruning, quantization, compression, and binary neural networks (BNNs), but with the emergence of the "extreme edge", there is now a demand for even more efficient models. In order to meet the constraints of ultra-low-energy devices, we propose ULEEN, a model architecture based on weightless neural networks. Weightless neural networks (WNNs) are a class of neural model which use table lookups, not arithmetic, to perform computation. The elimination of energy-intensive arithmetic operations makes WNNs theoretically well suited for edge inference; however, they have historically suffered from poor accuracy and excessive memory usage. ULEEN incorporates algorithmic improvements and a novel training strategy inspired by BNNs to make significant strides in improving accuracy and reducing model size. We compare FPGA and ASIC implementations of an inference accelerator for ULEEN against edge-optimized DNN and BNN devices. On a Xilinx Zynq Z-7045 FPGA, we demonstrate classification on the MNIST dataset at 14.3 million inferences per second (13 million inferences/Joule) with 0.21 $\mu$s latency and 96.2% accuracy, while Xilinx FINN achieves 12.3 million inferences per second (1.69 million inferences/Joule) with 0.31 $\mu$s latency and 95.83% accuracy. In a 45nm ASIC, we achieve 5.1 million inferences/Joule and 38.5 million inferences/second at 98.46% accuracy, while a quantized Bit Fusion model achieves 9230 inferences/Joule and 19,100 inferences/second at 99.35% accuracy. In our search for ever more efficient edge devices, ULEEN shows that WNNs are deserving of consideration.

==> background-old.tex <==

\subsection{Bloom Filters}
Although the WiSARD model avoids the state explosion problem inherent in large, simple WNNs, practical considerations still limit the sizes of the individual RAM nodes. Increasing the number of inputs to each RAM node will, up to a point, improve the accuracy of the model; however, the model size will also increase exponentially.
Fortunately, the contents of these large RAM nodes are highly sparse, as few distinct patterns are seen during in training relative to the large number of entries available. Prior work has shown that using hashing to map large input sets to smaller RAMs can greatly decrease model size at a minimal impact to accuracy\cite{Arajo2019MemoryEW}.

A Bloom Filter\cite{BloomFilter} is a hash-based data structure for approximate set membership. When presented with an input, a Bloom filter can return one of two responses: 0, indicating that the input is definitely not a member of the set, or 1, indicating that the element is \textit{possibly} a member of the set. False negatives do not occur, but false positives can occur with a probability that increases with the number of elements in the set and decreases with the size of the underlying data structure\cite{bloom_false_positive}.
Bloom filters have found widespread application for membership queries in areas such as networking, databases, web caching, and architectural predictions\cite{breternitz2008segmented}.
\revision{A recent model, Bloom WiSARD}\cite{Arajo2019MemoryEW}, demonstrated that replacing the RAM nodes in WiSARD with Bloom filters \revision{improves memory efficiency and model robustness} \cite{santiago2020weightless}.

Internally, a Bloom Filter is composed of $k$ distinct hash functions, each of which takes an $n$-bit input and produces an $m$-bit output, and a $2^{m}$-bit RAM.
%Each hash function takes an $n$-bit input and produces an $m$-bit output.
When a new value is added to the set represented by the filter, it is passed through all $k$ hash functions, and the corresponding bit positions in the RAM are set. When the filter is checked to see if a value is in the set, the value is hashed, and the filter reports the value as present only if all $k$ of the corresponding bit positions are set.
%A value is reported as present only if all $k$ of the bit positions corresponding to its hashed values are set. %A simple example of this is shown in Figure \ref{fig:bloom_filter}.

%\begin{figure}[hbtp]
%\centerline{\includegraphics[width = 0.8\columnwidth]{bloom_filter.png}}
%\caption{An example of a simple Bloom filter with $k=3$ hash functions. Hashed input $x_{1}$ corresponds to locations containing $\{1,0,1\}$, so produces an output of $0$ under the \texttt{AND} reduction. Hashed input $x_{2}$ corresponds to locations containing $\{1,1,1\}$, so produces an output of $1$.}
%\label{fig:bloom_filter}
%\end{figure}

\subsection{Bleaching}
Traditional RAM nodes activate when presented with any pattern they saw during training, even if that pattern was only seen once. This can result in overfitting, particularly for large datasets, a phenomenon known as \textit{saturation}. Bleaching \cite{bleaching} is a technique which prevents saturation by choosing a threshold $b$ such that nodes only respond to patterns they saw at least $b$ times during training. During training, this requires replacing the single-bit values in the RAM nodes with counters which track how many times a pattern was encountered. After training is complete, a bleaching threshold $b$ can be selected to maximize the accuracy of the network\footnote{Alternatively, $b$ may be chosen dynamically to serve as a tiebreaker when two or more discriminators produce an equal response. We do not explore this method of bleaching in this paper.}. 
Once $b$ has been selected, counter values greater than or equal to $b$ can be statically replaced with 1, and counter values less than $b$ with 0. Therefore, while additional memory is required during training, inference with a bleached WNN introduces no additional overhead.% This aligns with the paradigm of training on a large, central server and then deploying on edge devices.

In practice, bleaching can substantially improve the accuracy of WNNs. There have been several strategies proposed for finding the optimal bleaching threshold $b$; we use a binary search strategy based on the method proposed in \cite{bleaching}. Our approach performs a search between 1 and the largest counter value seen in any RAM node\revision{. Thus, both the space and time overheads of bleaching are worst-case logarithmic in the size of the training dataset.} %meaning that the number of bleaching values which are tested is worst-case logarithmic in the side of the training dataset.

\subsection{Thermometer Encoding}
Traditionally, WNNs represent their inputs as 1-bit values, where an input is 1 if it rises above some pre-determined threshold\footnote{Frequently the mean value of the input in the training data} and 0 otherwise. However, it is frequently advantageous to use more sophisticated encodings, where each parameter is represented using multiple bits\cite{wisard_encoding}. Integer encodings are not a good choice for WiSARD, since individual bits carry dramatically different amounts of information. In an 8-bit encoding, the most significant bit would carry a great deal of information about the value of a parameter, while the least significant bit would essentially be noise. Since the assignment of bits to RAM nodes is randomized, this would result in some inputs to some RAM nodes being useless.
%since the input order is randomized, and individual bits of multi-bit values carry different amounts of information. For instance, in an 8-bit binary encoding, the most significant bit carries a great deal of information about the value of a parameter, while the least significant bit is essentially noise.

In a thermometer encoding, a value is compared against a series of increasing thresholds, with the $i$'th bit of the encoded value representing the result of the comparison against the $i$'th threshold. Clearly if a value is greater than the $i$'th threshold, it is also greater than thresholds $\{0 \ldots (i-1)\}$; as Figure \ref{fig:thermometer} shows, the encoding resembles mercury passing the markings on an analog thermometer, with bits becoming set from least to most significant as the value increases. %This way, one has that both similarity and magnitude of values are preserved in this pattern representation.

\begin{figure}[hbtp]
\centerline{\includegraphics[width = 0.55\columnwidth]{figures/thermometer.pdf}}
\caption{Like the mercury passing the gradations in a thermometer, in a thermometer encoding, bits are set to 1 from least to most significant as the encoded value increases.}
\label{fig:thermometer}
\end{figure}
